See Your Heart: Psychological states Interpretation through Visual Creations

In psychoanalysis, generating interpretations to one's psychological state through visual creations is facing significant demands. The two main tasks of existing studies in the field of computer vision, sentiment/emotion classification and affective captioning, can hardly satisfy the requirement of psychological interpreting. To meet the demands for psychoanalysis, we introduce a challenging task, \textbf{V}isual \textbf{E}motion \textbf{I}nterpretation \textbf{T}ask (VEIT). VEIT requires AI to generate reasonable interpretations of creator's psychological state through visual creations. To support the task, we present a multimodal dataset termed SpyIn (\textbf{S}and\textbf{p}la\textbf{y} \textbf{In}terpretation Dataset), which is psychological theory supported and professional annotated. Dataset analysis illustrates that SpyIn is not only able to support VEIT, but also more challenging compared with other captioning datasets. Building on SpyIn, we conduct experiments of several image captioning method, and propose a visual-semantic combined model which obtains a SOTA result on SpyIn. The results indicate that VEIT is a more challenging task requiring scene graph information and psychological knowledge. Our work also show a promise for AI to analyze and explain inner world of humanity through visual creations.

==> record.tex <==
\begin{table*}[htb]
    \centering
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|}
        \hline
        Themes & Description & Examples \\
        \hline
        Energy & \makecell[l]{Alive, vital, intense energy is visible}  & \makecell[l]{Organic growth present, construction machines work \\on a task, airplanes take off from a runway}\\
        \hline
        Bridging & \makecell[l]{Connection between elements, joining of opposites}  & \makecell[l]{A ladder joins earth and tall trees; \\a bridge links an angel and devil }\\
        \hline
        Journeying & \makecell[l]{Movement along a path or around a center}  & \makecell[l]{A knight follows a trail;\\ a Native American paddles a canoe down a stream}\\
        \hline
        \makecell[c]{Going \\Deeper} & \makecell[l]{Discovery of a deeper dimension}  & \makecell[l]{A clearing is made, a treasure unearthed, a well dug,\\ a lake explored}\\
        \hline
        Spiritual & \makecell[l]{Religious or spiritual symbols present, such as\\ supernatural beings, worshipping figures \\or numinous items}  & \makecell[l]{Buddha overlooking newly married couple}\\
        \hline
        Chaotic & \makecell[l]{Haphazard, fragmented or formless arrangement}  & \makecell[l]{Objects flung into the tray, boundaries or \\outer reality disregarded, overall appearance ins \\jumbled/disconnected}\\
        \hline
        Empty & \makecell[l]{Reticence to use figures or lifeless feeling \\with lack of energy and curiosity}  & \makecell[l]{Nearly empty tray with only one dead tree \\placed in a corner}\\
        \hline
        Confined & \makecell[l]{Figure or groups normally free are entrapped or caged}  & \makecell[l]{An agonized figure is placed in a cage; a sand wall \\is built around an old woman}\\
        \hline
        Hindered & \makecell[l]{Possibility of new growth is impeded or hindered}  & \makecell[l]{A boat moving into new waters, while under siege \\by an army}\\
        \hline
    \end{tabular}
    }
    \caption{\textbf{Description and example of several themes.}}
    \label{table1}
\end{table*}





\begin{table}[thb]
    \centering
    %\resizebox{.95\columnwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
                                & \multicolumn{3}{l}{Accuracy} & FPR                & FNR                 \\
        \midrule
        \multirow{2}{*}{Total}  &\multirow{2}{*}{0.77} & Positive & 0.54              & \multirow{2}{*}{0.16} & \multirow{2}{*}{0.01}  \\
        \cline{3-4}
                                &                       & Negtive & 0.84              &                    &                     \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Sandplay work annotation result compare with SCL-90.} The accuracy include the positive accuracy(abnormal subjects accuracy), and negative accuracy(normal subjects accuracy). FPR means false positive rate, FNR means false negative rate.}
    \label{table2}
\end{table}



\section{3.2}
For the reason that human emotions are often metaphorical and complex, we do not directly utilize a specific emotion words to title each region, but utilize themes to classify regions, which is usually adapted by work in the field of psychology[][][]. Furthermore, the implication of a theme contains more semantic information than a single emotion word, which can help the model to have a stronger generalization when captioning the emotions. Our dataset categorized the regions into 24 themes, including Chaotic, Empty, Split, Confined, Neglected, Hidden, Prone, Injured, Threatened, Hindered, Rigid, Seeking Help, Bleak, Bridging, Journeying, Energy, Going Deeper, Birthing, Nurturing, Changed, Spiritual, Centered, Integrated, Praying. These 24 themes can be divided into two main categories, Wounding themes which cover the first 13 themes and Healing themes which cover the last 11 themes. The explanation of each theme is shown in Table 2. The distribution of each theme are shown in Table 3. The distribution of each theme regarding the sandplay regions is shown in Table 3.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.99\columnwidth]{theme_percent.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
    \caption{\textbf{Histogram of themems categorized in our dataset.}}
    \label{fig3}
\end{figure}



\subsection{2.1. Captioning models}
As the development of deep neural network, there are a lot of deep-net approaches for image captioning. We focused on apply several "standard" approaches on our dataset. Vinyals etc. introduced CNN plus LSTM network into image captioning. Anderson etc. introduced bottom up attention into image caption. Get rid of the CNN-LSTM structure, Cornia etc. gains a good result applying transformer structure into image captioning. Also, there are several reinforcement learning based method created for the exposure bias and undifferentiable metric problem of cross entropy method. For example, Rennie et al. proposed one of the most representative works in REINFORCE methods by using self-critical sequence training (SCST) to normalize the rewards and reduce the variance of the policy gradient.

A broad collection of methods have been proposed in the field of image captioning in the last few years. Earlier captioning approaches were based on the generation of simple templates, filled by the output of an object detector or attribute predictor[][]. With the development of Deep Neural Networks, image caption works started to use RNNs as language models and multilayer CNNs as visual information encoder[][][]. Based on the encoder-decoder models, there are also further improvements. One of the most important works is the bottom-up module which is proposed by Anderson et al. [] allowing the model dynamically focus on efficient features leading to learn better feature representations. However, such models face the problem of exposure bias[] and the mismatch between the optimizing function and the non-differentiable evaluation metrics, which lead to the notable achievement made by the introduction of Reinforcement Learning. Ranzato et al.[] firstly introduced REINFORCE algorithm to sequence training RNNs. To overcome the problem of the large variance of the policy gradient, many works have introduced different kinds of baseline into REINFORCE algorithm. Rennie et al. [] proposed one of the most representative works in REINFORCE methods by using self-critical sequence training (SCST) to normalize the rewards and reduce the variance of the policy gradient. In recent years, the Transformer architecture[] has made a great impact on modalities including both vision and language, even the image caption task have investigated Transformer-based models to overcome the limited representation power of RNN-based models. Transformer is an encoder-decoder model whose encoder and decoder parts both include a self-attention mechanism which has shew an effective result in multimodal applications. Huang et al. [] introduced a Transformer-like encoder to encode the regions into the hidden states, which was paired with an LSTM decoder. To effectively exploit both low-level and high-level contributions, Cornia et al.[] designed a encapsulates a multi-layer encoder for image regions and a multi-layer decoder which are connected mesh-like structure. Our work proposes baselines fit on our dataset mainly based on the classic and SOTA models mentioned above.

\subsection{2.2. Captioning datasets}
For a long time, researchers have devoted to the task of Image captioning as a bridge from vision to language, which has led a great deal of work on datasets in particular. Flickr 30K[] described each image with five independent sentence and Flickr 30K Entities[] annotated the nouns mentioned in the captions of Flickr30k by drew their bounding box in the image. Visual Genome[] and related previous efforts[][] provide short phrases describing regions in the images, which improved grounding to the phrase level. However, both in Flickr 30K Entities and Visual Genome, the bounding box partitions objects only, rather than a division partitioning the image into reasonable scenes or themes. In spite of this, their captions are confined to explicitly descriptions of objects without any intrinsic meanings about connections between objects or the emotional characteristic in the scene. One of the most broadly used dataset, MSCOCO[], tends to describe the picture as a whole in sentences and even has annotation on semantic segmentation. Nevertheless, the captions of MSCOCO is still explicit without any intrinsic meaning and the semantic segmentation can hardly combined with image captioning task. There are also works[] proposed captions in a form of paragraphs which stressed the context connection during describing the image. But the improve on language consistency may not bring the better partition of the scene or the intrinsic description of the image.

\subsection{2.3. Sentiment-driven captions}
There are particular rare work both involved emotion and image captioning. Mathews and follow-ups like [] are early works focused on injecting two emotions (positive and negative) into image captioning. They are works applied on real-world images which contains even zero creators emotion. The only two emotions injecting to the captioning is based on the visual cue through objective things without analyze of the scene. The recent work ArtEmis and its follow work [] proposed dataset combined emotional information and visual artworks. But the emotion information is the annotators' emotion reaction to the artwork but not focused on what the creator of the artworks want to express.








A broad collection of methods have been proposed in the field of image captioning in the last few years. Earlier captioning approaches were based on the generation of simple templates, filled by the output of an object detector or attribute predictor[][]. With the development of Deep Neural Networks, image caption works started to use RNNs as language models and multilayer CNNs as visual information encoder[][][]. Based on the encoder-decoder models, there are also further improvements. One of the most important works is the bottom-up module which is proposed by Anderson et al. [] allowing the model dynamically focus on efficient features leading to learn better feature representations.In recent years, the Transformer architecture[] has made a great impact on modalities including both vision and language, even the image caption task have investigated Transformer-based models to overcome the limited representation power of RNN-based models. Transformer is an encoder-decoder model whose encoder and decoder parts both include a self-attention mechanism which has shew an effective result in multimodal applications. Huang et al. [] introduced a Transformer-like encoder to encode the regions into the hidden states, which was paired with an LSTM decoder. To effectively exploit both low-level and high-level contributions, Cornia et al.[] designed a encapsulates a multi-layer encoder for image regions and a multi-layer decoder which are connected mesh-like structure. Our work proposes baselines fit on our dataset mainly based on the classic and SOTA models mentioned above.



\begin{table*}[b]
    \centering
    \resizebox{.95\textwidth}{!}{
    \begin{tabular}{lcccccccc}
        \toprule
        \multicolumn{1}{c}{Features} & BLEU-1 & BLEU-2 & BLEU-3 & BLUE-4 & ROUGE-L & METEOR & CIDEr-D & BERTScore-F1 \\
        \midrule
        (i) Visual features & 0.242 & 0.127 & 0.086 & 0.064 & 0.288 & 0.121 & 0.482 & 0.678 \\
        + (ii) scene graph information only & 0.261 & 0.152 & 0.109 & 0.089 & 0.319 & 0.132 & 0.671 & 0.694 \\
        + (iii) psychological knowledge only & 0.239 & 0.136 & 0.102 & 0.078 & 0.295 & 0.129 & 0.632 & 0.688  \\
        + (iv) S\&K both & \textbf{0.295} & \textbf{0.170} & \textbf{0.122}  & \textbf{0.095}   & \textbf{0.335} & \textbf{0.150} & \textbf{0.874} & \textbf{0.711} \\
        \bottomrule
    \end{tabular}
    }
\caption{\textbf{Alation study results.} We combine different extra information with visual features. S\&K both means that both scene graph information and psychological knowledge information are combined.}
\label{table4}
\end{table*}
